The Entropy Power Inequality and Mrs. Gerber's Lemma for Abelian Groups of Order 2^n

Shannon's Entropy Power Inequality can be viewed as characterizing the minimum differential entropy achievable by the sum of two independent random variables with fixed differential entropies. The entropy power inequality has played a key role in resolving a number of problems in information theory. It is therefore interesting to examine the existence of a similar inequality for discrete random variables. In this paper we obtain an entropy power inequality for random variables taking values in an abelian group of order 2^n, i.e. for such a group G we explicitly characterize the function f_G(x,y) giving the minimum entropy of the sum of two independent G-valued random variables with respective entropies x and y. Random variables achieving the extremum in this inequality are thus the analogs of Gaussians in this case, and these are also determined. It turns out that f_G(x,y) is convex in x for fixed y and, by symmetry, convex in y for fixed x. This is a generalization to abelian groups of order 2^n of the result known as Mrs. Gerber's Lemma.

==> applications_sec7.tex <==
\section{Applications}
Hereafter we will refer to random variables taking values on $\mathbb{Z}_{2^n}$ as $2^n$-ary random variables.
\subsection{Scalar and Vector MGL}
\begin{claim}\label{scalarMGL}
Let $X$, $Y$ and $Z$ be  $2^n$-ary random variables and let $U$ be an arbitrary random variable. Suppose $Z$ is independent of $(U,X)$ and $Y = X + Z$ where the addition is understood to be the group addition. Then
$$H(Y|U) \geq f_{2^n}(H(X|U),H(Z))$$
\end{claim}
\begin{remark}
In the case of binary random variables where $Z \sim Bern(p)$, the scalar MGL is given by 
$$H(Y|U) \geq H(H^{-1}(H(X|U)) \star p)$$
Thus, Claim \ref{scalarMGL} can be thought of the scalar MGL for $2^n$-ary random variables. 
\end{remark}
\begin{proof}[Proof of Claim \ref{scalarMGL}]
\begin{align}
H(Y|U) &= \sum_{u} P(U=u)H(Y|U=u)\\
&= \sum_{u}P(U=u)H(X+Z|U=u)\\
&\geq \sum_{u}P(U=u)f_{2^n}(H(X|U=u),H(Z)) \label{scalarMGL3}\\
& \geq f_{2^n} \left( \sum_{u} P(U=u)H(X|U=u), H(Z)\right) \label{scalarMGL4}\\
&= f_{2^n}(H(X|U),H(Z))
\end{align}
where (\ref{scalarMGL3}) follows from the definition of $f_{2^n}$ and (\ref{scalarMGL4}) follows from the convexity of $f_{2^n}$
\end{proof}

\begin{claim}\label{vectorMGL}
Let $X^n$ be a $2^k$-ary random vector and $U$ be an arbitrary random variable. If $Z^n$ is a vector of independent identically distributed $2^k$-ary variables, distributed according to $p_Z$, independent of $(X^n, U)$ and $Y^n = X^n + Z^n$ then
$$\frac{H(Y^n|U)}{n} \geq f_{2^k} \left( \frac{H(X^n|U)}{n}, H(Z) \right) $$
\end{claim}
\begin{remark}
Claim \ref{vectorMGL} in the case of binary random variables where $Z^n$ is a vector of iid random variables having distribution Bern($p$), is given by
$$\frac{H(Y^n|U)}{n} \geq H \left(H^{-1}\left( \frac{H(X^n|U)}{n}\right) \star p \right) $$
Thus, Claim \ref{vectorMGL} can be thought of as the vector MGL for $2^n$-ary random variables.
\end{remark}
\begin{proof}[Proof of Claim \ref{vectorMGL} ]

\begin{align}
\frac{H(Y^n|U)}{n} &= \sum_{i=1}^{n} \frac{H(Y_i|U, Y^{i-1})}{n}\\
& \geq \sum_{i=1}^{n} \frac{H(Y_i|U, Y^{i-1},X^{i-1})}{n} \label{vectorMGL2}\\
&= \sum_{i=1}^{n} \frac{H(Y_i|U, X^{i-1})}{n} \label{vectorMGL3} \\
& \geq \sum_{i=1}^{n} \frac{ f_{2^n}(H(X_i | U, X^{i-1}), H(Z))}{n} \label{vectorMGL4}\\
& \geq  f_{2^n} \left( \sum_{i=1}^{n}\frac{H(X_i | U, X^{i-1})}{n}, H(Z)\right) \label{vectorMGL5}\\
&= f_{2^n}\left( \frac{H(X^n | U)}{n}, H(Z) \right)
\end{align}
Here, (\ref{vectorMGL2}) is because conditioning reduces entropy, (\ref{vectorMGL3}) is because the channel from $X^n$ to $Y^n$ is a DMC, (\ref{vectorMGL4}) follows from the scalar MGL, (\ref{vectorMGL5}) is because of the convexity of $f_{2^n}$.
\end{proof}

\subsection{Degraded broadcast channels}

We'll now consider a class of degraded broadcast channels and arrive at a simple expression for computing its capacity region. The motivation behind this is the capacity region expression of the binary symmetric broadcast channel (BS-BC). Consider a  BS-BC with input $X$ and outputs $Y_1,Y_2$ where $X$ to $Y_1$ is BSC($p_1$) and $X$ to $Y_2$ is BSC($p_2$) and w.l.o.g. $p_1 < p_2 < \frac{1}{2}$. Its capacity region given by
\begin{align*}
R_1 &\leq H(\alpha \star p_1) - H(p_1)\\
R_2 &\leq 1 - H(\alpha \star p_2)\\
\end{align*}
for some $\alpha \in [0,\frac{1}{2}]$. This region is achievable using superposition coding. We will recall the converse here. Let $Z_1 \sim$ Bern($p_1$) and $Z_2 \sim$ Bern($p_2$). We can take $Y_1= X + Z_1$ and $Y_2 = X+Z_2$. Now note that a BS-BC is stochastically degraded since we can write
$Y_2 = X + Z_1 + \tilde{Z_2}$ where $\tilde{Z_2} \sim$ Bern$\left(\frac{p_2-p_1}{1-2p_1}\right)$. The capacity of a degraded broadcast channel is given by
\begin{align*}
R_1 &\leq I(X,Y_1 | U)\\
R_2 &\leq I(U; Y_2)\\
\end{align*}
over all $U - X - (Y_1,Y_2)$.   We have 
$$I(U; Y_2) = H(Y_2) - H(Y_2|U) \leq 1 - H(Y_2| U)$$
Since $1 \geq H(Y_2|U) \geq H(Y_2|X) = H(p_2)$, there exists $\alpha \in [0, \frac{1}{2}]$ such that $H(Y_2|U) = H(\alpha \star p_2)$. Next consider 
$$I(X;Y_1|U) = H(Y_1|U) - H(Y_1|X) = H(Y_1|U) - H(p_1)$$
Now by the scalar MGL, we have 
$$H(Y_2 | U) = H(Y_1 + \tilde{Z_2}|U) \geq H(H^{-1}(H(Y_1|U)) \star \tilde{p_2})$$
But $H(Y_2 | U) = H( \alpha \star p_2) = H(\alpha \star p_1 \star \tilde{p_2})$. This implies
$$H(Y_1 | U) \leq H(\alpha \star p_1)$$ 
and thus
$$I(X;Y_1|U) \leq H(\alpha \star p_1) - H(p_1)$$
proving the converse. 
\smallskip

Now suppose we try to adapt this converse to the case of a degraded $2^n$-ary broadcast channel, with the two channels having noise $Z_1$, $Z_2$ and $Z_2 \sim Z_1  + \tilde{Z_2}$. Let the distributions be $Z_1 \sim p_{Z_1}$, $Z_2 \sim p_{Z_2}$ and $\tilde{Z_2} \sim p_{\tilde{Z_2}}$. We have
$$I(U,Y_2) = H(Y_2) - H(Y_2 | U) \leq n - H(Y_2|U)$$
Since $n \geq H(Y_2 | U) \geq H(Y_2 | X) = H(p_{Z_2})$, there exists a $p_\alpha$ such that $H(Y_2 | U) = H(p_\alpha \circledast p_{Z_2})$. Next consider 
$$I(X;Y_1|U) = H(Y_1|U) - H(Y_1|X) = H(Y_1|U) - H(p_{Z_1})$$
Now by the scalar MGL, we have 
$$H(Y_2 | U) \geq f_{2^n}(H(Y_1|U), H(p_{\tilde{Z_2}}))$$
Thus we have
$$H(p_\alpha \circledast p_{Z_1} \circledast p_{\tilde{Z_2}}) \geq  f_{2^n}(H(Y_1|U), H(p_{\tilde{Z_2}}))$$
From this we wish to conclude that $H(p_\alpha \circledast p_{Z_1} ) \geq H(Y_1 | U)$. Notice that if we had
$$f_{2^n}(H(p_\alpha \circledast p_{Z_1} ), H(p_{\tilde{Z_2}})) \geq f_{2^n}(H(Y_1|U), H(p_{\tilde{Z_2}}))$$
we would get what we want. This leads us to conclude that if we had the equality
\begin{equation}\label{f=h}
H(p_\alpha \circledast p_{Z_1} \circledast p_{\tilde{Z_2}}) = f_{2^n}(H(p_\alpha \circledast p_{Z_1} ), H(p_{\tilde{Z_2}}))
\end{equation}
which essentially means that $p_\alpha \circledast p_{Z_1}$ and $p_{\tilde{Z_2}}$ should be a pair of equality achieving distributions for $f_{2^n}$. Consider the class of broadcast channels where $p_{\tilde{Z_2}}$ is such that it takes constant values on the cosets of $\mathbb{Z}_{2^{n-1}}$ (we shall refer to such distributions as $2^n$-ary Gaussian henceforth) and $p_{Z_1}$ is arbitrary. We know that $p_{\tilde{Z_2}}$ is an optimizing distribution. Note also that since $p_{Z_2} = p_{Z_1} \circledast p_{\tilde{Z_2}}$, $p_{Z_2}$ is also a $2^n$-ary Gaussian. This means we can choose $p_\alpha$ to be $2^n$-ary Gaussian as well. With this choice of $p_\alpha$, we note that $p_\alpha \circledast p_{Z_1}$ is now $2^n$-ary Gaussian and thus (\ref{f=h}) holds. We can now make the following claim:
\begin{claim}\label{bc2n}
The capacity of a $2^n$-ary degraded broadcast channel where $\tilde{Z_2}$ is a $2^n$-ary Gaussian is given by
\begin{align*}
R_1 &\leq H(p_\alpha)-H(p_{Z_1})\\
R_2 &\leq n - H(p_\alpha \circledast p_{Z_2})\\
\end{align*}
for some $2^n$-ary Gaussian distribution $p_\alpha$.
\end{claim}
\begin{proof}[Proof of Claim \ref{bc2n}]
The achievability follows from superposition coding, and the converse follows from the preceding discussion.
\end{proof}
\begin{corollary}\label{cor_bc2n}
If both $Z_1$ and $Z_2$ are $2^n$-ary Gaussian, the capacity of the corresponding broadcast channel is given by
\begin{align*}
R_1 &\leq H(p_\alpha \circledast p_{Z_1})-H(p_{Z_1})\\
R_2 &\leq n - H(p_\alpha \circledast p_{Z_2})\\
\end{align*}
where $p_\alpha$ can be chosen from a suitable family of distributions $\{p_\alpha\}$ which satisfies the property:  for every $x \geq H(p_{Z_2})$, there exists an $p_{\alpha_0} \in \{p_\alpha\}$ such that $H(p_{\alpha_0} \circledast p_{Z_2}) = x$.
\end{corollary}
\begin{remark}
Choosing $\{p_\alpha\}$ to be the family of $2^n$-ary Gaussian distributions satisfies the property.
\end{remark}
\begin{proof}[Proof of Corollary \ref{cor_bc2n}]
If both $Z_1$ and $Z_2$ are $2^n$-ary Gaussian, it is clear the the broadcast channel is degraded and $p_{\tilde{Z_2}}$ can be taken to be a $2^n$-ary Gaussian distribution. In the converse, we see that regardless of what $p_\alpha$ is, $p_\alpha \circledast p_{Z_1}$ will always be $2^n$-ary Gaussian because $Z_1$ is $2^n$-ary Gaussian. Thus so long as we can find a suitable $p_\alpha$,  (\ref{f=h}) will continue to hold and the converse remains true.
\end{proof}


\subsection{Lossless source coding with helper}

If $(X,Y)$ is a 2-DMS, the optimal rate region for lossless source coding of $X$ with a helper observing $Y$ is the set of rate pairs $(R_1,R_2)$ such that
\begin{align*}
R_1 & \geq H(X|U)\\
R_2 & \geq I(Y;U)\\
\end{align*}
for some conditional pmf $p(u|y)$. In the case of a DSBS($p$), $p \in [0, \frac{1}{2}]$ the optimal rate region expression simplifies to 
\begin{align*}
R_1 & \geq H(\alpha \star p)\\
R_2  & \geq 1 - H(\alpha)\\
\end{align*}
The achievability of this region follows from taking the $U$ to $Y$ channel as a BSC($\alpha$). We'll go through the proof of the converse and try to adapt it to a class of double symmetric $2^n$-ary sources.\\
Since $H(X|Y) = H(p) \leq H(X|U) \leq 1$, there exists $\alpha \in [0, \frac{1}{2}]$ such that $H(X|U) = H(p \star \alpha)$. By the scalar MGL, $H(X|U) = H(Y+Z|U) \geq H(H^{-1}(H(Y|U)) \star p)$. Thus we have $H(\alpha \star p) \geq H(H^{-1}(H(Y|U)) \star p)$, giving $\alpha \geq H^{-1}(H(Y|U))$. This implies
\begin{align*}
I(Y;U) &= H(Y) - H(Y|U)\\
&= 1 - H(Y|U)\\
& \geq 1 - H(\alpha)
\end{align*}
proving the converse. 
\smallskip

Now consider a DS-$2^n$-ary source $(X,Y)$ such that $Z \sim p_Z$. We have $H(X|Y) = H(p_Z) \leq H(X|U) \leq n$, thus there exists a $p_\alpha$ such that $H(X|U) = H(p_Z \circledast p_\alpha)$. By the scalar MGL, $H(X|U) \geq f_{2^n}(H(Y|U), H(Z))$, that is $H(p_Z \circledast p_\alpha) \geq f_{2^n}(H(Y|U), H(Z))$. From this we want to conclude that 
$$H(p_\alpha) \geq H(Y|U)$$
Note that if we had 
$$f_{2^n}(H(p_\alpha), H(p_Z)) \geq f_{2^n}(H(Y|U), H(Z))$$ 
we would be able to conclude this. This means that we should have 
$$H(p_Z \circledast p_\alpha) = f_{2^n}(H(p_\alpha), H(p_Z))$$
Now if $Z$ is a $2^n$-ary Gaussian, we can choose $p_\alpha$ to be a $2^n$-ary Gaussian as well, giving the equality above. We can thus make the claim
\begin{claim}\label{sourcehelper}
Let $(X,Y)$ be a doubly symmetric $2^n$-ary source such that $X = Y + Z$ where $Z$ is  $2^n$-ary Gaussian distributed as $p_Z$. The optimal rate region for lossless source coding of $X$ with a helper observing $Y$ is the set of rate pairs $(R_1,R_2)$ such that 
\begin{align*}
R_1 &\geq H(p_\alpha \circledast p_Z)\\
R_2 &\geq n - H(p_\alpha)\\
\end{align*}
for some $2^n$-ary Gaussian $p_\alpha$.
\end{claim}
\begin{proof}[Proof of Claim \ref{sourcehelper}]
The achievability follows from taking $Y$ to $U$ to have noise $\sim p_\alpha$ and the converse follows from the preceding discussion.
\end{proof}


%\section{Modulo $2^n$ sum relay channel}
%\begin{claim}\label{relay2n}
%Consider the discrete memoryless relay channel (DM-RC) in Figure \ref{relay} where
%$$Y_3' = X_1 + Z_3$$
%$$Y_2 = Z_2 + Z_3$$
%where $Z_2$ is $2^n$-ary Gaussian and $Z_3$ is uniform, both independent of each other and of $X_1$. For $C_0 \in [0,n]$, the capacity of this relay channel is 
%$$C = 1 - f_{2^n}(H(Z_2), n-C_0)$$
%\end{claim}

%\begin{proof}[Proof of Claim \ref{relay2n}]
%We have the compress-forward lower bound for a DM-RC orthogonal receiver components from \cite{gamal_kim_11} 
%$$C \geq \max_{p(x_1),p(\hat{y_2}|y_2)} \min \{I(X_1;Y_3') - I(Y_2; \hat{Y_2}; X_1,Y_3') +C_0, I(X_1; \hat{Y_2}, Y_3')\}$$
%Let $p_\alpha$ be $2^n
%\end{proof}















==> z4_sec3_inprelim.tex <==
\begin{lemma}\label{concavity}
$f(x,y)$ is concave along lines thought the origin, i.e. $f(x,\theta x)$ is concave in $x$ for $0 \leq \theta \leq \infty$, and strictly concave for $0 < \theta < \infty$
\end{lemma}
\begin{proof}[Proof of Lemma \ref{concavity}]
When $\theta = 0$ or $\infty$, $f(x,y)$ is linear, thus concave. For $0 < \theta < \infty$, by Lemma \ref{dfdx}, we have that $\frac{\partial f}{\partial x}$ decreases along lines though the origin. By symmetry, it follows that $\frac{\partial f}{\partial y}$ also decreases along lines through the origin. Since
\begin{equation}
\frac{df(x,\theta x)}{dx} =  \frac{\partial f}{\partial x} + \theta  \frac{\partial f}{\partial y}
\end{equation}
it is immediate that $\frac{df(x,\theta x)}{dx}$ also decreases along the line of slope $\theta$, which means that $f(x,\theta x)$ is strictly concave.

\end{proof}

\begin{lemma} \label{unique}
If  $(x_1,y_1), (x_2,y_2) \in (0,\log2)\times(0,\log2)$ and $(\frac{\partial f}{\partial x} ,\frac{\partial f}{\partial y})\bigg|_{(x_1,y_1)} = (\frac{\partial f}{\partial x} ,\frac{\partial f}{\partial y})\bigg|_{(x_2,y_2)}$ then $(x_1,y_1)=(x_2,y_2)$
\end{lemma}
\begin{remark}
The above lemma says that in the interior of the unit square, the pair of partial derivatives at a point uniquely determine the point. That this fails on the boundary is seen from the fact that for any point of the form $(x,0)$ the pair of partial derivatives evaluates to be $(1,0)$ and for every point of the form $(0,y)$ it is $(0,1)$.
\end{remark}
\begin{proof}[Proof of Lemma \ref{unique}]
Without loss of generality, assume $x_1 \leq x_2$. We consider two cases: $y_1 \geq y_2$ or $y_1 < y_2$.\\ Suppose $y_1 \geq y_2$, in this case we have
\begin{equation}
\frac{\partial f}{\partial x}\bigg|_{(x_1,y_1)} \leq \frac{\partial f}{\partial x}\bigg|_{(x_2,y_1)} \leq  \frac{\partial f}{\partial x}\bigg|_{(x_2,y_2)}
\end{equation}
The first inequality follows from Mrs. Gerber's Lemma. To see the why the second is true, recall the expression  
\begin{align}
\frac{\partial f}{\partial x} =& \frac{\partial f}{\partial p}  \frac{\partial p}{\partial x}\\
=&(1-2q)\log\left(\frac{1-p \star q}{p \star q}\right) \times \frac{1}{\log\left(\frac{1-p}{p}\right)}
\end{align}
Thus for a fixed $p$, as $q$ increases $\frac{\partial f}{\partial x}$ strictly decreases. Note also that atleast one of the two inequalities is strict as $(x_1,y_1) \neq (x_2,y_2)$. Thus
\begin{equation}\label{ineq1}
\frac{\partial f}{\partial x}\bigg|_{(x_1,y_1)} < \frac{\partial f}{\partial x}\bigg|_{(x_2,y_2)}
\end{equation}
Inequality ($\ref{ineq1}$) implies that $y_1 \geq y_2$ cannot hold, and it must be that $y_1 < y_2$. We can also assume $x_1 < x_2$, since $x_1 = x_2$   combined with $y_1 < y_2$ gives 
$$\frac{\partial f}{\partial x}\bigg|_{(x_1,y_1)} > \frac{\partial f}{\partial x}\bigg|_{(x_2,y_2)}$$
The only remaining case is thus $(x_1,y_1) < (x_2,y_2)$. Consider the line passing through the origin and $(x_1,y_1)$. We again break this up into two cases: either $y_2 \geq x_2 \frac{y_1}{x_1}$ or  $y_2  \leq x_2 \frac{y_1}{x_1}$.  \\
If  $y_2 \geq x_2 \frac{y_1}{x_1}$, 
\begin{equation}
\frac{\partial f}{\partial x}\bigg|_{(x_1,y_1)} > \frac{\partial f}{\partial x}\bigg|_{(x_2, x_2 \frac{y_1}{x_1})} \geq  \frac{\partial f}{\partial x}\bigg|_{(x_2,y_2)}
\end{equation}
Where the first inequality follows from Lemma \ref{dfdx}, and the second follows from $\frac{\partial f}{\partial x}$ decreasing for a fixed $x$ and an increasing $y$.\\
If   $y_2  \leq x_2 \frac{y_1}{x_1}$, we have
\begin{equation}
\frac{\partial f}{\partial y}\bigg|_{(x_1,y_1)} > \frac{\partial f}{\partial y}\bigg|_{(y_2\frac{x_1}{y_1}, y_2)} \geq  \frac{\partial f}{\partial y}\bigg|_{(x_2,y_2)}
\end{equation}
Where the first inequality follows from Lemma \ref{dfdx} and the fact that $y_2\frac{x_1}{y_1} > x_1$. The second inequality follows from the symmetric analogue of $\frac{\partial f}{\partial x}$ decreasing for a fixed $x$ and an increasing $y$, which is that $\frac{\partial f}{\partial y}$ decreases for a fixed $y$ and an increasing $x$.. This completes the proof of Lemma \ref{unique}.


\end{proof}



